Decentralized Control of Uncertain Multi-Agent Systems with Connectivity Maintenance and Collision Avoidance

This paper addresses the problem of navigation control of a general class of uncertain nonlinear multi-agent systems in a bounded workspace of $\mathbb{R}^n$ with static obstacles. In particular, we propose a decentralized control protocol such that each agent reaches a predefined position at the workspace, while using only local information based on a limited sensing radius. The proposed scheme guarantees that the initially connected agents remain always connected. In addition, by introducing certain distance constraints, we guarantee inter-agent collision avoidance, as well as, collision avoidance with the obstacles and the boundary of the workspace. The proposed controllers employ a class of Decentralized Nonlinear Model Predictive Controllers (DNMPC) under the presence of disturbances and uncertainties. Finally, simulation results verify the validity of the proposed framework.

==> procedure_flow.tex <==
% Define block styles
\tikzstyle{decision} = [diamond, draw, %fill=blue!20,
    text width=7.5em, text badly centered, node distance=3cm, inner sep=0pt]
\tikzstyle{block} = [rectangle, draw, %fill=blue!20,
    text width=7em, text centered, minimum height=4em]
\tikzstyle{line} = [draw, -latex']
\tikzstyle{cloud} = [draw, ellipse, %fill=red!20,
    node distance=3cm, minimum height=4em, minimum width=4em]

\begin{tikzpicture}[node distance = 2cm, auto]
    % Place nodes
    \node [decision] (decide) {Current configuration feasible?};
    \node [cloud, below of=decide, node distance=5.5cm] (stop) {stop};

    \node [block, right of=decide, node distance=5cm] (solve_1) {Agent 1: solve FHOCP and apply control input};
    \node [block, below of=solve_1, node distance=2.5cm] (solve_2) {Agent 2: solve FHOCP and apply control input};
    \node [block, below of=solve_2, node distance=3cm] (solve_N) {Agent N: solve FHOCP and apply control input};

    \node [block, right of=solve_1, node distance=5cm] (solve_1_) {Agent 1: solve FHOCP and apply control input};
    \node [block, below of=solve_1_, node distance=2.5cm] (solve_2_) {Agent 2: solve FHOCP and apply control input};
    \node [block, below of=solve_2_, node distance=3cm] (solve_N_) {Agent N: solve FHOCP and apply control input};


    \node [above of=decide, node distance=3cm] (step_0) {STEP 0};
    \node [above of=solve_1, node distance=3cm] (step_1) {STEP 1};
    \node [above of=solve_1_, node distance=3cm] (step_1_) {STEP 2};


    % invisible nodes
    \node[inner sep=0,minimum size=0,right of=solve_N, node distance=2.5cm] (sN) {};
    \node[inner sep=0,minimum size=0,left of=solve_1_, node distance=2.5cm] (s1_) {};
    \node[inner sep=0,minimum size=0,right of=solve_N_, node distance=2.5cm] (sN_) {};
    \node[inner sep=0,minimum size=0,right of=solve_1_, node distance=2.5cm] (s1_inv) {};
    \node[right of=solve_1_, node distance=3.5cm] (solve_1_inv) {$\dots$};


    \path [line]        (decide)  -- node {NO}(stop);
    \path [line]        (decide)  -- node {YES}(solve_1);
    \path [line]        (solve_1) -- node {}(solve_2);
    \path [line,dashed] (solve_2) -- node {}(solve_N);
    \path [line]        (solve_1_) -- node {}(solve_2_);
    \path [line,dashed] (solve_2_) -- node {}(solve_N_);

    \path [line] (solve_N) -- (sN);
    \path [line] (sN) -- (s1_);
    \path [line] (s1_) -- (solve_1_);

    \path [line] (solve_N_) -- (sN_);
    \path [line] (sN_) -- (s1_inv);
    \path [line] (s1_inv) -- (solve_1_inv);

\end{tikzpicture}

